A Scalable Actor-based Programming System for PGAS Runtimes

The PGAS model is well suited for executing irregular applications on cluster-based systems, due to its efficient support for short, one-sided messages. However, there are currently two major limitations faced by PGAS applications. The first relates to scalability: despite the availability of APIs that support non-blocking operations in special cases, many PGAS operations on remote locations are synchronous by default, which can lead to long-latency stalls and poor scalability. The second relates to productivity: while it is simpler for the developer to express all communications at a fine-grained granularity that is natural to the application, experiments have shown that such a natural expression results in performance that is 20x slower than more efficient but less productive code that requires manual message aggregation and termination detection. In this paper, we introduce a new programming system for PGAS applications, in which point-to-point remote operations can be expressed as fine-grained asynchronous actor messages. In this approach, the programmer does not need to worry about programming complexities related to message aggregation and termination detection. Our approach can also be viewed as extending the classical Bulk Synchronous Parallelism model with fine-grained asynchronous communications within a phase or superstep. We believe that our approach offers a desirable point in the productivity-performance space for PGAS applications, with more scalable performance and higher productivity relative to past approaches. Specifically, for seven irregular mini-applications from the Bale benchmark suite executed using 2048 cores in the NERSC Cori system, our approach shows geometric mean performance improvements of >=20x relative to standard PGAS versions (UPC and OpenSHMEM) while maintaining comparable productivity to those versions.

==> background.tex <==

\subsection{Actor/Selector}
The Actor Model~\cite{actor,actors_agha} is an asynchronous message-based concurrency model. The key idea behind actors is to encapsulate mutable state and to use asynchronous messaging to coordinate activities among actors. The actor runtime maintains a separate logical mailbox for each actor. Any actor or non-actor, can send messages to an actor's mailbox.  An actor also maintains a local state, which is initialized during creation.
%The actor is only allowed to update its local state using data from the messages it receives.
The actor is restricted to process at most one message at a time, thereby avoiding data races and the need for synchronization. In the actor model, there is no restriction on the order in which the actor processes incoming messages. %though many implementations (including ours) preserve the order of messages received from the same sender.
Selector~\cite{shams_selector} is an extension of actor with multiple mailboxes.

%In summary, actors can send and receive messages to and from other actors. Non-actors can send messages to actors, but cannot receive messages.  The sending and receiving of messages is performed asynchronously, i.e. the sending actor can deliver a message without waiting for the receiving actor to be ready to process the message.

%\subsection{Selector}
%An actor cannot control the order in which messages are processed and this can make it challenging to implement synchronization and coordination patterns. This issue is addressed by introducing an extension to the actor model called selectors~\cite{shams_selector}. Selectors have multiple mailboxes, and each mailbox is guarded i.e., it can be enabled or disabled to affect the order in which messages are processed. Similar to an actor, a selector is defined as an object that has the capability to process incoming messages. Selectors continue to encapsulate their local state and process one message at a time. Thus the benefits of modularity from the actor model are still preserved, and the data locality properties of the actor model continue to hold.

%\subsection{Message Aggregation Libraries}
%Message aggregation is a communication optimization technique that aggregates a set of small messages into a single large message to achieve higher communication bandwidth. Such optimization is not only well suited to regular dense applications but also to irregular applications in which every single PE (processing element) makes numerous point-to-point updates/gets to/from a random distributed location.

\subsection{HClib Asynchronous Many-Task (AMT) Runtime} \label{sec:hclib}
\input{hclib}











==> motivation.tex <==
In this section, we discuss productivity-performance trade-offs inherent in  the use of message aggregation libraries, and discuss our motivation for building a selector-based programming system. We use Conveyors~\cite{conveyors} as a primary exemplar of a message aggregation library because it is state-of-the-art, modular, portable, highly efficient, frugal with memory, and scalable to very large systems. However, our approach is applicable to other message aggregation libraries as well.

Conveyors~\cite{conveyors} is a C-based message aggregation library built on top of conventional communication libraries such as SHMEM, MPI, and UPC. It provides the following three basic operations:
\begin{enumerate}
	\item \texttt{push} (\texttt{convey\_push}): attempts to enqueue a message for delivery to a specified PE.
	\item \texttt{pull} (\texttt{convey\_pull}): attempts to receive a message (including which PE sent it).
	\item \texttt{advance} (\texttt{convey\_advance}): which ensures forward progress of communication.
\end{enumerate}

It is worth noting that both \texttt{push} and \texttt{pull} operations can fail. \texttt{push} can fail due to a lack of buffer space, and \texttt{pull} can fail due to a lack of an available item. Due to these failures, \texttt{push} and \texttt{pull} operations must always be placed in a loop that calls \texttt{advance} to ensure progress and to also detect termination.  Calling \texttt{advance} too frequently can result in extra overheads, while failing to call \texttt{advance} when needed
can result in deadlock.

To set the context for this section, we  discuss two essential communication idioms commonly found in distributed irregular applications, namely \textit{update} and \textit{gather} idioms.  Since the focus of our work in on scalable parallelism, 
we assume that each processing element (PE) executes the same code
in the following code examples  (as in the SPMD model).

\subsubsection{Idiom 1: Update Pattern}
This pattern is used extensively in computations where each PE needs to update a local or remote location that is only known dynamically at the time of the update.
A simple PGAS version of this pattern is shown in \autoref{lst:histogram_agi}.
This program creates a histogram in a distributed array named \texttt{histo} based on global indices stored in each PE's local \texttt{index}  array (\texttt{+} performs an atomic increment).  
%It was obtained from the Bale~\cite{bale} suite of mini-applications, where the ``AGI''  versions in \texttt{apps/*/*\_agi.*} are intended to showcase coding patterns that are natural to PGAS programmers.
As can be seen in \autoref{lst:histogram_agi}, this version supports 
a ``global view'' of the single distributed \texttt{histo}  array. The corresponding operation can be done in OpenSHMEM using \texttt{shmem\_int64\_atomic\_add/inc}, UPC using \texttt{upc\_atomic\_relaxed} and MPI using \texttt{MPI\_Accumulate/Get\_Accumulate/Fetch\_and\_op}.

\begin{comment}
\begin{lstlisting}[caption={An example program that creates a histogram by updating a distributed array.}, label={lst:histogram_agi}, escapechar=|]
  for(i = 0; i < n; i++) {
    histo[index[i]] += 1
\end{lstlisting}
\end{comment}

\begin{lstlisting}[caption={An example program that creates a histogram by updating a distributed array.}, label={lst:histogram_agi}, escapechar=|]
  for(i = 0; i < n; i++) {
    spot = index[i] / PROCS;
    PE = index[i] % PROCS;
    shmem_atomic_inc(histo+spot, PE);
\end{lstlisting}

The Conveyors version of this pattern from the Bale suite is shown in \autoref{lst:histogram_conv}.
This version is based on ``local views'', in which each PE has a local array, 
\texttt{histo}, and the set of local arrays implicitly defines a distributed global array based on a cyclic (round-robin) distribution of global array elements across the PEs.

\begin{lstlisting}[caption={An example program that uses Conveyors to create a histogram by updating a distributed array\cite{conveyors}.}, label={lst:histogram_conv}, escapechar=|]
  convey_begin(c);
  int i = 0, spot;
  while (convey_advance(c, i == n)) { |\label{line:histo_advance}|
     for (; i < n; i++) {
       spot = index[i] / PROCS; |\label{line:histo_c_loc}|
       PE = index[i] % PROCS;  |\label{line:histo_c_pe}|
       if(!convey_push(c, &spot, PE)) |\label{line:histo_push}|
         break;
     }
     while (convey_pull(c, &spot, &from)) |\label{line:histo_pull}|
       histo[spot]++;
  }
\end{lstlisting}

In Lines~\ref{line:histo_c_loc} and \ref{line:histo_c_pe}, since \texttt{histo} is distributed in a  round-robin fashion, the executing PE rank first finds a target array location (\texttt{spot}) and a target PE rank (\texttt{PE}). Then, in Line~\ref{line:histo_push}, the executing PE attempts to enqueue the location for delivery to the target PE. After that, in Line~\ref{line:histo_pull}, the executing PE attempts to retrieve a set of messages that have been sent from other PEs, and perform the desired updates (increments) in accordance with those messages. Two important points to note are: 1) no atomic operation is required since all updates to any location are done by the one PE with affinity to that location, and 2) since both \texttt{convey\_push} and \texttt{convey\_pull} operations can fail, they are enclosed in \texttt{if} or \texttt{while} statements to check for false return values. In case of failure, \texttt{convey\_advance} is called to perform an actual communication, and this cycle is repeated until all the items are pushed (\texttt{i == n}) and all communications are completed. As shown in \autoref{tab:motivation}, the Conveyors version is an order of magnitude faster than other versions on 2048 PEs (64 nodes with 32 core per node i.e., one PE per core) in the Cori supercomputer (details on the performance evaluation methodology are presented later in \autoref{sec:evaluation}).

\subsubsection{Idiom 2: Gather Pattern}
The second common idiom is the \textit{gather} pattern, in which each PE sends a request for  data from a random distributed location and then processes the data received in response to the request. An AGI version of a program using this pattern is shown in \autoref{lst:ig_agi} (also taken from the Bale suite). This program reads data from a distributed array named \texttt{data} (``global view'') and stores the retrieved values in a local array named \texttt{gather} based on global indices stored in a local array named \texttt{index}. The corresponding operation can be done in OpenSHMEM using \texttt{shmem\_int64\_g} or \texttt{shmem\_int64\_get\_nbi} , UPC as shown in the listing or using \texttt{upc\_memget\_nbi} and MPI using \texttt{MPI\_Get}.

\begin{lstlisting}[caption={An example program that reads data from a distributed array.}, label={lst:ig_agi}, escapechar=|]
for(i = 0; i < n; i++) {
  gather[i]=data[index[i]];
\end{lstlisting}

Compared to the \textit{update} pattern, the \textit{gather} pattern involves both \textit{to} and \textit{from} communications. Specifically, each PE first makes a request to a target PE for a specific value (data[index[i]]), which needs to be sent back to the requester PE.  In contrast, there was no need for a response to the requester PE  in the \textit{update} pattern. Due to this two-way communication, a performant implementation of the \textit{gather} pattern requires two Conveyors, one for querying the location and another for sending back the responses. A Conveyors version of this pattern from the Bale suite is shown in \autoref{lst:ig_conv}. As in the Conveyors version of the Update Pattern, we assume ``local views'', in which each PE has a local array, 
\texttt{data}, and the set of local arrays implicitly defines a distributed global array based on a cyclic (round-robin) distribution of global array elements across the PEs.

\begin{lstlisting}[caption={An example program that uses Conveyors to gather data from a distributed array\cite{conveyors}.}, label={lst:ig_conv}, escapechar=|]
struct packet { long slot; long value; } pkt;
int i = 0, from;
bool more;
convey_begin(q); convey_begin(r); 

while (more = convey_advance(q, i == n),    |\label{line:ig_advance1}|
            more OR convey_advance(r, !more)) {  |\label{line:ig_advance2}|
   for (; i < n; i++) {
      pkt.slot = i;
      pkt.value = index[i] / PROCS;
      PE = index[i] % PROCS
      if (! convey_push(q, &pkt, PE))   |\label{line:ig_pushq}|
         break;
   }
   while (convey_pull(q, &pkt, &from)) { |\label{line:ig_pullq}|
      pkt.value = data[pkt.value];
      if (! convey_push(r, &pkt, from)) { |\label{line:ig_pushr}|
         convey_unpull(q);  |\label{line:ig_unpull}|
         break;
      }
   }
   while (convey_pull(r, &pkt, &from)) |\label{line:ig_pullr}|
      gather[pkt.slot] = pkt.value;
}

\end{lstlisting}

The two conveyors, \texttt{q} and \texttt{r}, are coupled together in that conveyor \texttt{q} is used for sending and  processing queries and conveyor \texttt{r}  is used for sending and  processing responses.
%it does not look like a simple composition of the two Conveyors.
The array location that needs to be accessed is sent to the PE that owns that portion of the array at Line~\ref{line:ig_pushq}. The target PE pulls this query at Line~\ref{line:ig_pullq} and processes it. While processing the query, it gets the value from the \texttt{data} array and returns this value to the requester using \texttt{convey\_push} in Line~\ref{line:ig_pushr}. One important detail that needs to be addressed is what to do if this \texttt{convey\_push} fails. The natural solution is to save the packet from the failed push to some temporary storage and process it again later. To help with this, the Conveyors library provides the  \texttt{convey\_unpull} convenience method through which we can put the packet back to where it was taken from, as shown in Line~\ref{line:ig_unpull} so that it can be processed again later. Finally, the PE that requested the remote data receives it in Line~\ref{line:ig_pullr} and stores it in the \texttt{gather} array. As shown in \autoref{tab:motivation}, the Conveyors version beats all other versions by a handsome margin on 2048 PEs (with one PE per core) in the Cori supercomputer.

%For completeness, \autoref{tab:motivation} also shows the performance of a version of this benchmark using OpenSMHEM non-blocking \texttt{get} operations (with a call to \texttt{shmem\_quiet()} for termination), and we see that it takes more than twice the execution time of the Conveyors version.
%Further, non-blocking gets/puts are limited in their use, and cannot (for example) 
%be used to implement the histogram mini-application since OpenSHMEM does not provide non-blocking interfaces for remote atomics.  The main reason for including this data point was to show that the Conveyors library performs better than OpenSHMEM nonblocking operations for the Index Gather mini-application.

Although the performance and scalability of the Conveyors based implementations is excellent, the programs are neither easy to write nor easy to understand. The application programmer has to take care of error-handling operations as well as retry operations that are interleaved with \texttt{advance} operations. These complexities place a significant burden on programmer productivity and assumes a high expertise level. A good alternative to improve performance would be to include such high-performance message aggregation libraries underneath the current non-blocking communication mechanisms in OpenSHMEM/UPC/MPI. However, \autoref{tab:motivation} demonstrates that user-assisted message aggregation can achieve much higher performance compared to automatic message aggregation~\cite{upc_aggr1,upc_aggr2} performed by non-blocking operations in the state of the art communication systems.

Although Histogram and Index-gather can be easily converted from the trivial blocking versions to their non-blocking versions, it is not necessarily true for many other applications. ~\autoref{lst:triangle_snippet} shows a code snippet from a triangle counting application where data is used as soon as they are accessed from the remote locations. The non-blocking version of such applications results in code complexity significantly higher compared to their blocking equivalents. Even with such higher complexity, the non-blocking versions would not be able to achieve performance anywhere close to a version written using a performant user-initiated message aggregation library based on our results from ~\autoref{tab:motivation}. This points to a direction that implies the current non-blocking communication interfaces are not the best abstraction for message aggregation, and therefore we decided to explore a better abstraction.

\begin{lstlisting}[caption={A small UPC code snippet from triangle counting application that uses data from distributed locations.}, label={lst:triangle_snippet}, escapechar=|]
...
int64_t kbegin = L->offset[L_j];  //Remote
int64_t kend    = L->offset[L_j + THREADS]; //Remote
numpulled+=2;
for( kk = kbegin; kk < kend; kk++){
	w = L->nonzero[ L_j%THREADS + kk*THREADS]; //Remote
	numpulled++;
	for(ii = start; ii < L->loffset[l_i + 1]; ii++) {
		if( w ==  L->lnonzero[ii] ){
		...
\end{lstlisting}

Targeting user-initiated message aggregation libraries by application programmer is not a scalable approach even though it provides very high performance. There could be multiple such libraries, each with a different interface. This brings in the need for a higher-level abstraction that can perform on par with the message aggregation libraries. The actor model is a good candidate for such an abstraction since the mailbox provides a natural facility to aggregate messages.  Although not extensively used in HPC, the actor model has been in existence for a while and used as a primary concurrency mechanism in languages such as Scala and Erlang. Therefore Actors can provide a more standardized interface compared to individual message aggregation libraries.

This motivates us to address the following research question:

\noindent\textbf{Research Question}: \textit{What is a desirable intermediate point in the productivity-performance space, 1) with scalable performance that approaches close to high performance aggregation libraries (such as Conveyors) and 2) with productivity that is higher compared to such libraries?}

\begin{table}[t]
\centering
\begin{tabular}{|l|l|l|l|}
\hline
                              &             & NB &Time \\ \hline
\multirow{2}{*}{Histogram}    & OpenSHMEM   (cray-shmem 7.7.10)      &  Y & 4.3         \\ \cline{2-4}
                              & UPC  (Berkley-UPC 2020.4.0) & Y &  23.9         \\ \cline{2-4}
                              & MPI3-RMA (OpenMPI 4.0.2)   & Y &88.9         \\ \cline{2-4}
                              & MPI3-RMA (cray-mpich 7.7.10)   & Y &$>$300         \\ \cline{2-4}
                              & Charm++ (6.10.1,  gni-crayxc w/ TRAM)  & Y & 9.7         \\ \cline{2-4}
                              & Conveyors (2.1 on cray-shmem 7.7.10)  & Y & 0.5         \\ \hline
\multirow{2}{*}{IndexGather} & OpenSHMEM   (cray-shmem 7.7.10)     & N     & 35.5        \\ \cline{2-4}
							 & OpenSHMEM NBI  (cray-shmem 7.7.10)           &  Y &4.2        \\ \cline{2-4}
                              & UPC (Berkley-UPC 2020.4.0) & N &22.6  \\ \cline{2-4}
                              & UPC NBI (Berkley-UPC 2020.4.0) & Y & 19.7 \\ \cline{2-4}
                              & MPI3-RMA (OpenMPI 4.0.2)   & Y & 25.8         \\ \cline{2-4}
                              & MPI3-RMA (cray-mpich 7.7.10)   & Y & 8.3         \\ \cline{2-4}
                              & Charm++ (6.10.1,  gni-crayxc w/ TRAM)  & Y & 21.3         \\ \cline{2-4}
                              & Conveyors (2.1 on cray-shmem 7.7.10)   & Y & 2.3         \\ \hline
\end{tabular}
\caption{Absolute performance numbers in seconds using best performing variants for Histogram and Index Gather on 2048 PEs (64 nodes) in the Cori supercomputer which performs 2$^{23}$ ($\approx$ 8 million, changed due to charm++ memory issue) updates for Histogram and reads for Index Gather. Each version is annotated with a non-blocking (NB) specifier.}
\label{tab:motivation}
\end{table}

In \autoref{sec:design} and \autoref{sec:impl}, we discuss how the use of the selector model addresses this research question.


==> non_blocking.tex <==

We know from \autoref{tab:motivation} that the non-blocking operations in standard communication libraries such as OpenSHMEM are slower compared to message aggregation libraries such as Conveyors. Therefore, one way to accelerate OpenSHMEM is to add message aggregation from scratch or use existing libraries such as Conveyors. Since our Actor/Selector runtime provides comparable performance to Conveyors, we added a proof of concept implementation (included in the artifact) of two OpenSHMEM non-blocking operations using the Actor/Selector interface, thereby adding message aggregation capabilities to them. We added \texttt{shmem\_get\_nbi} so as to implement the read pattern benchmark and \texttt{shmem\_atomic\_inc} to implement the update pattern benchmark used in~\autoref{sec:motivation}. To put in perspective, if we extend \autoref{tab:motivation} with this message aggregation supported OpenSHMEM operations, the time taken for the Read benchmark is 2.5 sec, and that of Update benchmark is 0.5 sec which is the same as the Actor/Selector version. Implementing all the non-blocking OpenSHMEM operations is future work since the topic of this paper is to create a scalable Actor based programming system rather than conventional non-blocking communication routines.

